Miriam: Exploiting Elastic Kernels for Real-time Multi-DNN Inference on Edge GPU

Many applications such as autonomous driving and augmented reality, require the concurrent running of multiple deep neural networks (DNN) that poses different levels of real-time performance requirements. However, coordinating multiple DNN tasks with varying levels of criticality on edge GPUs remains an area of limited study. Unlike server-level GPUs, edge GPUs are resource-limited and lack hardware-level resource management mechanisms for avoiding resource contention. Therefore, we propose Miriam, a contention-aware task coordination framework for multi-DNN inference on edge GPU. Miriam consolidates two main components, an elastic-kernel generator, and a runtime dynamic kernel coordinator, to support mixed critical DNN inference. To evaluate Miriam, we build a new DNN inference benchmark based on CUDA with diverse representative DNN workloads. Experiments on two edge GPU platforms show that Miriam can increase system throughput by 92% while only incurring less than 10\% latency overhead for critical tasks, compared to state of art baselines.

==> backup/new-5-backup.tex <==
\section{Runtime Dynamic Kernel Coordination}
% \vspace{-1ex}
\begin{figure}[t!]%[htb]
\centering
\includegraphics[scale=1.4]{image_bk/mcoordmar8.pdf}
\caption{Shaded Binary Tree Construction for Kernel Shards Formations in the critical mode. ES refers to the elastic kernel, and EBS refers to the elastic block size. The sharding degree represents the degree of elastic kernel splitting depth.}
\label{binary}
\end{figure}

% DNN Indepodence =>  
% To achieve the high throughput of normal tasks while preserving the low latency of co-running critical tasks. The generated elastic kernels for normal tasks should be only served using the leftover GPU resources from kernels of critical tasks without leading to severe resource contention. Although static kernel fusion can merge multiple kernels launched on different GPU streams into one fused kernel to reach time-multiplexing, however, there can be thousands of fragments consisting in an elastic DNN kernel, which makes this approach unpractical. For example, .....
We introduce our design of our coordinator in this section, the online scheduler for elastic kernel coordinations. The guidelines are two-fold: to maximize the overall system performance, and to mitigate resource contention. 

The runtime coordinator monitors the current GPU resources left over by the critical kernels and determines the elastic kernel shards that co-running with critical kernels.



\noindent\textbf{Execution timeline of co-running kernels.} Miriam provides two DNN inference modes at runtime: the \textit{Critical Mode} and the \textit{Normal mode}. Upon receiving multiple normal tasks requests $b1...bn$, Miriam runs in the normal mode, all the kernels are pushed into the normal tasks queue and are dispatched to the GPU semantic through multiple streams. Miriam will switch from this mode to the critical mode once a critical task arrives. Miriam will instantly select appropriate elastic kernel fragments of the following normal kernel in a "bin-packing" manner, considering the current intra- and inter-SM-level resource distributions.  After that, once the critical kernels finished executing, all the kernels from normal tasks will re-occupying the GPU. 

%neiwen: story line of section 6
%1. Execution timeline of co-running kernels (phases) : how to launch kernels + timeline explaination
%2. Grid/block determination:how to determine grid and block for elastic kernel
%3. dynamic elastic kernel formation: how to construct the overall shaded kernel binary tree

% Another key challenge is that: The online scheduler module should be lightweight. Otherwise, the overhead itself can result in the d eadline missing critical tasks. Is it possible to adopt more heuristics instead of the computation-based predictor (e.g. MLP-based predictor) to assist the kernel coordination? In this section, we propose \textit{MCoord}, the kernel coordinator working at runtime.

\noindent\textbf{Key Challenges for grid/block size determination of elastic kernels. }
During runtime, a fixed size for elastic grids and block settings for elastic kernels can easily become inefficient with the optimal co-scheduled elastic kernel shards varying with different co-running with critical kernels. For example, if one critical kernel finishes and there still exists half of the computations unfinished from the co-locating elastic kernel, the rest half of thread blocks from it lead to severe resource contention or underutilization when co-locating with the subsequent critical kernel. 

The elastic kernel fragment selection policy is important to avoid latency interference with critical tasks, which selects a set of shards from candidate normal kernels to share the GPU with the arriving critical kernels. Optimally, we need to precisely predict the isolated inference time for normal kernels and the inference time when co-locating them with elastic kernel shards. Some readers may ask if we can use the runtime performance events (e.g., cache misses, global memory bandwidth) and the inherent features of the operators as the inputs to build a duration model for operator groups \cite{orion, horus} formation. The fact is that edge GPUs such as Nvidia Jetson devices do not provide any interfaces to obtain runtime events online. The hardware events reported by tools like nisght-sys and nsight-compute can only be obtained statically \cite{nsys} or retrieved with a register inside SMs with high overhead\cite{reef}. It is not applicable to rely on these hardware events to build the model for the online kernel coordinations. 


\noindent\textbf{Dynamic shaded binary tree construction. }We propose a dynamic-sized shade binary tree approach for elastic kernel shards formation to achieve high runtime efficiency and low resource contention according to dynamic arrived critical DNN tasks.

The shaded binary tree structure is an abstract for managing the elastic kernel shards, which is similar to a complete binary tree structure of shards, as is shown in Fig. \ref{binary}. The root of the tree represents the kernel from the normal tasks, whose initial grid size is $M$. Each node corresponds to a part of computations, or potential thread blocks to be dispatched inside the kernel. The shading property for each node is the elastic block size of the thread block. Directed edges  indicate the potential sliced peers for the unfinished computations left over from the predecessor. The whole structure is composed of the actual shard and the virtual shard. The actual shards are the ultimately formed elastic kernel shards that are to be dispatched, and the virtual shards are the potential fragments of the elastic kernel that would not be dispatched.

Miriam relies on the dynamic shaded kernel binary tree structure to manipulate the elastic kernels from normal tasks and determines the elastic kernel shards with heuristics based on the number of thread blocks of kernels from both critical and normal tasks. As is shown in fig. \ref{binary}, which illustrates the life cycle of an elastic normal kernel. For elastic fragment selection from normal kernels, the policy is to pick a set of elastic blocks from the head of the shaded kernel binary tree to share SM-level resources with co-locating thread blocks from resident critical kernels with trivial contention. Miriam proposes to utilize a  policy to ensure that the elastic blocks from normal kernels will only use the left-over resources from the critical kernels.





%% This declares a command \Comment
%% The argument will be surrounded by /* ... */




% \begin{algorithm}[!ht]
% \DontPrintSemicolon
  
% \KwInput{Your Input}
% \KwOutput{Your output}
% \KwData{Test set $x$}
% $\sum_{i=1}^{\infty} := 0$ \tcp*{this is a comment}
% \tcc{Now this is an if...else conditional loop}
% \If{Condition 1}
% {
%     Do something    \tcp*{this is another comment}
%     \If{sub-Condition}
%     {Do a lot}
% }

% \ElseIf{Condition 2}
% {
%     Do Otherwise \;
%     \tcc{Now this is a for loop}
%     \For{sequence}    
%     { 
%         loop instructions
%     }
% }

% \Else
% {
%     Do the rest
% }
    
% \tcc{Now this is a While loop}
% \While{Condition}
% {
%    	Do something\;
% }

% \caption{The details of \textit{MCoord} Scheduler}
% \end{algorithm}

==> backup/new-6-backup.tex <==
\section{Addition Optimization} \label{addition}
At the end-to-end DNN inferences pipeline, there includes two steps before and after the computations for the kernel on the GPU: bidirectional memory copies between the host (CPU) and the device (GPU), which can be implemented in CUDA via APIs such as $cudaMemcpyAsync(H2D,D2H)$. We can overlap the kernel execution as well as the data transfer and thus minimize the time consumption for data by using a stream for asynchronous launching \cite{cudaoverlap}. The asynchronous behavior of kernel launches from the host’s perspective makes the overlapping device and host computation convenient. 

For some DNN models that contain unstructured operators (e.g. $op.transpose$ in the $MultiheadAttention$ layer of the transformer model \cite{mobilevit}), the degree of their potential parallelism is dynamic and hard to predict. It is naturally difficult to equally divide tasks into blocks and threads, resulting in unbalanced load and performance problems. Miriam will adopt the \textit{Dynamic Parallelism Principles (DPP)} (e.g. Cuda Dynamic Parallelism (CDP) \cite{cdp}) towards these operators if the compiler-generated or handwritten GPU kernels do not consider the optimizations. Specifically, the launched kernels with DPP handle the parallel computation workload that is discovered dynamically by a parent thread at runtime, and the parent threads only have to issue a child kernel that handles the parallel computation with little or no control divergence. During the compilation stage, Miriam only takes into consideration of the initial kernel for end-to-end transformation  and leaves the modeling of all nodes in the nested parallelism to future work.



==> bk.tex <==
\section{BK} 

% \begin{figure}[t!]%[htb]
% \centering
% \includegraphics[width=0.48\textwidth]{image_sysdesign/systemdesign.pdf}
% \caption{Miriam system design.}
% \label{fig:sys}
% \end{figure}

==> framework.tex <==
\section{Introduction}
% e story logic in my head: if we want to improve
% average-case throughput, then has to increase resource uti-
% lization, so has to live with the complex and unpredictable
% contentions, so cannot achieve good real-time performance;
% on the other hand, to achieve good real-time performance by
% forbidding contention lead to poor throughput. What to do if
% the system has real-time and throughput requirements at the
% same time? The key is to be able to ’control’ the contention
% somehow, so that the desired real-time performance of those
% critical tasks is guaranteed, while the remaining resource can
% be utilized by other tasks as much as possible to maximize
% their throughput. However, ’control’ the contention is chal-
% lenging due to the mixed and complex factors (because there
% is no way to control how the kernel access the resources). We
% propose Miriam to achieve this. The main idea of Miriam is to
% transform the kernels into elastic kernels, the resource access
% of which can be changed and controlled at runtime, according
% to the current need

\section{Background and Motivation Study}
\textbf{LOGIC:} multi-DNN inference on edge GPU everywhere -> Real-time requirements and throughput requirements -> Unavoidable and complex resource contention, e2e latency high -> if manually forbidden contention, throughput low ->motivation: obtain an appropriate distribution of SM resources among co-executing kernels.
\subsection{Terminology}
\subsection{Characterization of multi-DNN Inferences on Edge GPU}
Launch inference tasks in kernel sequences via GPU stream.
\subsection{Complex Resource Contention of Concurrent Kernels}
unpredictable kernel overlap.
\subsection{Unstable Latency and End-to-end Throughput of Inference Tasks}
Resource underutilization if manually forbids contention.
\subsection{Unbalanced workloads across SMs in GPU [DO WE NEED?]}

\section{Problem Formulation}
4.2 critical ? normal
\section{Miriam Overview}
\subsection{Key Idea}
propose elastic kernel, what is? how to? Usage?
\subsection{System Architecture}
Introduce each component in Miriam at a high level(offline transformation -> online coordination) 
\section{Generation of Elastic Kernels}
(Design of elastic kernels->How to generate?)
Two dimensions: elastic grid, block. End-2-end transformation. Design Space. Relationship between elastic kernel => elastic grid<>elastic block  
\subsection{Controllable Intra-SM Resource by Elastic Block}
: Improving Intra-SM Parallelism

\subsection{Kernel Slicing based on Elastic Grid}
Reducing Inter-SM Resource Contention

\subsection{Consolidation of the Two Elastic Dimensions [DO WE NEED?]}

\subsection{Narrowing Down Design Space}

\subsection{Source-to-Source Kernel Transformer}

\section{Dynamic Kernel Coordination}
How can we use elastic kernels?

\noindent\textbf{Execution timeline of co-running kernels.}

\noindent\textbf{Key Challenges for grid/block size determination of elastic kernels.}

\noindent\textbf{Dynamic shaded binary tree construction.}
\section{Additional Optimizations}
1). Pipeline for memory copy and computation.
2). Dynamic parallelism for unstructured kernels. 
\section{Implementations}
\section{Experiments}





==> new_10discussion_bk.tex <==
\section{Discussion} \label{discussion}
\subsection{}
\noindent\textbf{Complementary as Machine Learning Compiler Runtime}
\subsection{Orthogonal to Other Optimizations}
\noindent\textbf{Working with NAS and Model Compression.}
Miriam works with model compression.




Miriam can serve as post-processing middle-ware for ML Compilers.

\noindent\textbf{Supporting Collaborative Inference on Heterogeneous Platforms}
Miriam supports cross-device optimizations.
\cite{hem}

\subsection{Finer-grained GPU Multitasking Management}
Warp-level resource management may bring improvement, however, the potential overhead risks would also be larger.
\subsection{Extending Miriam to Other Platforms}

%\vspace{-2.2ex}
\section{Conclusion}
In this work, we introduce Miriam, a DL optimization \& runtime framework for mixed-critical DNN workloads on edge GPU.

==> new_2problem.tex <==
\vspace{-1em}
\section{Design Goal and Principle} \label{problem}
% This paper considers the impact of co-locating multiple DNN inference tasks on edge GPUs in real-time scenarios. Latency-critical tasks, referred to as critical tasks in this paper, have strict real-time requirements and include tasks such as obstacle detection in autonomous driving \cite{ecrt}. In contrast, normal tasks with no hard real-time requirement, referred to as normal tasks in this paper, can also be co-located on the edge GPU. Examples of normal tasks include driver facial recognition.
Miriam considers co-running DNN inference tasks on edge GPU for real-time applications. We define critical tasks in this paper as tasks that have strict real-time requirements. For example, obstacle detection in autonomous driving must be finished by a certain deadline, allowing sufficient time for the vehicle to maneuver around obstructions. Otherwise, it could potentially pose safety risks to the driver.
For other tasks that have no hard real-time performance, we define them as normal tasks in our paper. For example, monitoring human drivers' emotions and fatigue needs to be executed in a best-effort manner to improve the driving experience.
%in-car speech recognition tasks xxxx need to be executed in time xxx to improve the xxxx.
%such as obstacle detection in autonomous driving \cite{ecrt,reef}. For other tasks that have no hard real-time performance which is expected to be executed in a best-effort manner, we define it as normal tasks in our paper, for example, in-car speech recognition tasks need to be executed in time to improve 

\sysname{} aims to meet the real-time requirement for latency-critical tasks while maximizing the overall throughput of co-running normal tasks in a dynamic manner. 
%DNN sequences from all the arrival tasks, both latency-critical and normal, are in a random pattern. 
Given two incoming DNN task queues for \textit{normal task $\tau^{normal{}}$} and \textit{critical task $\tau^{critical{}}$}. We aim to find a policy at runtime that can minimize the execution time of normal tasks while guaranteeing the real-time performance of critical tasks. 
%The problem can be formulated as:
\setlength{\belowdisplayskip}{2pt}
\setlength{\abovedisplayskip}{2pt}
% \begin{equation}
% \begin{aligned}
% \pi^{*} = argmin\  Latency(\tau^{normal{}}_{\pi}), \pi\in\Pi \, \, \, \, \, s.t. \\ 
% Latency(\tau^{critical{}}_{\pi^{*}})<\alpha*Latency(\tau^{critical{}}_{solo}) 
% % Cost(\pi)<\beta
% \end{aligned}
% \end{equation}


% \begin{equation}
% \begin{aligned}
% \pi^{*} = \mathop{\arg\min}\limits_{L(\tau^{critical{}}_{\pi^{*}}) \to L(\tau^{critical{}}_{solo}) }  L(\tau^{normal{}}_{\pi}), \pi\in\Pi 
% % Cost(\pi)<\beta
% \end{aligned}
% \end{equation}

% 多目标优化：尽可能pareto front，尽可能dominant;不应该选critical最小的pareto，选这个点因为收益比～
% 设计哲学：in general是一个多目标优化问题 -> 【首先pf, 其次选取哪个点作为目标】-> 有很多design choice，递进选哪个点 -> 配个概念图示意一下 = 只付出一点点critical latency的代价就能收获大量throughput benefits. critical task SOLO clearly, 设计哲学，一起扔进去contention complex，

% a * latency() 换成 绝对值参数constraint, 
% 实验里ddl，solo*slowdown来设置。
% a* -> 
% 接近于1
% 

%where $Latency(*)$ is the measured execution latency of DNN tasks. $Latency(\tau_{solo})$ is the end-to-end latency of the tasks while they are running in a solo manner, and $\alpha$ here represents a coefficient that limits the maximized acceptable speed loss of the critical tasks. $\pi$ is our designed execution strategy which will be introduced in Section~\ref{system}.
%$\pi$ is the strategy for elastic kernel selection policy for normal kernels and coordination for co-running kernels (i.e., critical and normal kernels). We will illustrate the definitions of the elastic kernels we proposed in Section 3.

%To summarize, the goal of Miriam is to minimize the end-to-end latency for normal tasks while preserving the inference speed of critical tasks. 

==> new_6addition.tex <==
% \vspace{-1em}
\section{Addition Optimization} \label{addition}
% At the end-to-end DNN inferences pipeline, there includes two steps before and after the computations for the kernel on the GPU: bidirectional memory copies between the host (CPU) and the device (GPU), which can be implemented in CUDA via APIs such as $cudaMemcpyAsync(H2D,D2H)$. We can overlap the kernel execution as well as the data transfer and thus minimize the time consumption for data by using a stream for asynchronous launching \cite{cudaoverlap}. The asynchronous behavior of kernel launches from the host’s perspective makes the overlapping device and host computation convenient. 
{\color{blue}
For some DNN models that contain unstructured operators (e.g. $op.transpose$ in the $MultiheadAttention$ layer of the transformer model \cite{mobilevit}), the degree of their potential parallelism is dynamic and hard to predict. It is naturally difficult to equally divide tasks into blocks and threads, resulting in unbalanced load and performance problems. Miriam adopts the \textit{Dynamic Parallelism Principles (DPP)} (e.g. Cuda Dynamic Parallelism (CDP) \cite{cdp}) towards these operators if the compiler-generated or handwritten GPU kernels do not consider the optimizations. Specifically, the launched kernels with DPP handle the parallel computation workload that is discovered dynamically by a parent thread at runtime, and the parent threads only have to issue a child kernel that handles the parallel computation with little or no control divergence. During the compilation stage, Miriam only takes into consideration of the initial kernel for end-to-end transformation and leaves the modeling of all nodes in the nested parallelism to future work.

}

==> new_7implementation.tex <==
\section{Implementation} \label{implementation}

\begin{table}[]
\caption{Implementation Specifications}
\centering
\scalebox{0.72}{
\begin{tabular}{c|c}
\hline
Hardware   & \begin{tabular}[c]{@{}c@{}}Desktop GPU: GTX 2060 (34 SMs); \\ Edge GPU: Jeston Orin (16 SMs); Jeston Xaiver (8 SMs)\end{tabular} \\ \hline
Software   & CUDA Version: 11.2; Jetpack Version: 4.5; TVM Version: 0.9                                                                       \\ \hline
DNN Models & \begin{tabular}[c]{@{}c@{}}ResNet18; AlexNet; GRU; LSTM; CifarNet; \\ TVM Compiled ViT; TVM Compiled Inception\_v3\end{tabular}  \\ \hline
\end{tabular}
}
\label{implement:1}
\end{table}

We implemented Miriam based on CUDA 11.2 for elastic kernel generation and online kernel scheduling, python3.6 for kernel transformer. Specifically, We deployed Miriam on NVIDIA GTX 2060, Jetson Orin and Jetson Xaiver. CUDA multi-stream is enabled to allow concurrent execution of GPU kernels. Specifically, 


==> new_9related_bk.tex <==

\section{Related Work} \label{related}
We compare and contrast Miriam with prior works in the following three aspects: on-device DNN inference serving, multi-DNN coordination system and multi-tasking on GPU.

\subsection{On-device DNN Inference Serving}
On-device DNN inference in full-stack can be roughly expanded in input data level, DNN kernel level, DNN model level, and hardware resource level. Works such as \cite{elf,edgeluyang} either adopts content-aware inputs selection mechanisms or heat-map-based processing of input streams algorithms to improve on-device inference efficiency; Model-level optimization has been extensively studied to exploit the sparsity of DNN models, e.g., iterative pruning \cite{lottery} and neural network search \cite{nas}; Kernel-level optimizations can be categorized into single-tenant DNN compiling techniques \cite{TVM,TASO}, which generate high-performance tensor programs inside each DNN kernel, or automatically find the optimal kernel fusion \cite{nimble} and parallelism strategy to accelerate the end-to-end DNN inference speed \cite{iosmlsys}. Some compiler-level works such as Rammer \cite{rammer} and TensorRT \cite{tensorrt} enable both inter- and intra-operator parallelism for accelerating DNN inference. Some recent works also exploit to utilize heterogeneous platforms \cite{dart, codl} e.g. mobile CPU \& GPU to boost inference performance. Dart \cite{dart} proposes a pipeline-based approach to co-run diverse DNN workloads on heterogeneous computation nodes. As mentioned, most of these works rapidly degrade under multi-DNN inference settings due to severe resource contention. Our work focuses on improving multi-DNN inference serving on a single edge GPU.
% Our work focuses on edge GPU, which have emerged as a popular accelerator to serve DNN inferences for edge computing applications \cite{gpu good}. As mentioned, directly running multiple DNN tasks concurrently on a single edge GPU will result in severe latency degradation which may exceed the QoS target set by users due to on-board resource contention.

\subsection{DNN Compiling}
Although most vendor-provided libraries such as NVIDIA cuDNN offer optimized DNN kernels with convenient APIs (e.g. $cudnn\_conv\_winograd$), many researchers have put their attention on DNN compilers, which automatically generate high-performance kernels which outperform those libraries. Although traditional DNN compilers such as IOS,  TVM and XLA \cite{iosmlsys,TVM,xla} have extensively explored either graph substitution based on inter-operator parallelism \cite{astitch} or kernel optimization \cite{rammer} based on intra-operator parallelism to boost inference speed. Unfortunately, they mainly target at optimizing one model under static environments, which is ill-fitted for mutli-DNN inference scenarios,s and give no consideration to on-device resource contentions on edge devices. For example, Auto-scheduler in Ansor \cite{ansor}, as Figure \ref{background1} shows, for a GEMM kernel on a RTX2060 GPU, the tuned configurations are aimed to saturate all SMs and memory bandwidth on the GPU, while these configurations can be sub-optimal when there are only partial resources available for the task when there comes another DNN task. The latency gap between single-model vs. multi-models with different tuned configurations can be X difference for a GEMM kernel. 

Readers may raise the question why not try leveraging DNN compilers to generate multiple versions of kernels under different contention levels, and adapt them online, switch the version of kernels in order to avoid resource contention? There are two main drawbacks of this kind of approach, current popular learning-based DNN compilers such as TVM search the optimal code transformation during compiling, leading to extremely long search time. For example, the time consumption for on-device measurements of a VGG16 model can be up to 10 hours on an NVIDIA TX2 \cite{moses}, which is unacceptable, not to say to generate multiple versions of a single kernel. Besides, pre-loading multiple versions of kernels into GPU will be a memory disaster. Thus, we cannot directly apply DNN compiler to solve the problem.

\subsection{Multi-DNN Coordination System}
A number of systematic solutions have been proposed in order to solve the on-device multi-DNN coordination problem, which can be divided into two categories: \textit{compression-enabled DNN inference system} and \textit{runtime operator scheduling system}. As for the prior one, works like NestDNN \cite{nestdnn} and RT-mDL \cite{rt-mdl} leverage DNN model compression techniques to provide a multi-variants design for each DNN model and to enable on-device multi-DNN inference acceleration by trading accuracy of each model at a modest level to exhaustively reduce the computation demands of the incoming mixed DNN workloads \cite{modelcompression}. There exist two main drawbacks: first, the compression ratio is task-dependent which makes the system less generality. Second, the model complexity-efficiency trade-off of these compressed models is determined in advance and is fixed after deploying them online, leading to rigid adaptiveness to varying runtime on-board resources. There are representative works for the second direction such as DeepEye \cite{deepeye}, Abacus \cite{enablesc} and Dart \cite{dart}. The key idea behind these works is to interleave operators with different "contention channels" (memory-bound or compute-bound) to avoid on-device resource contention, and thus to coordinate different DNN inference tasks. However, these works suffer from a time-consuming offline profiling process and are hard to generalize to new incoming DNN tasks. Above all, all these mentioned works can be described as \textit{"contention inhibitors"}, which deal with the multi-tasks on-device contention problems with an evasive attitude. Although it partially solves the contention by avoiding it, it would easily lead to resource under-utilization. Miriam consolidates both \textit{"contention inhibitors"} and \textit{"Contention Incentives"} to maximize on-device parallelism and minimize contention brought by multi-DNN inference on edge GPU.

\subsection{GPU Multi-tasking}
Current popular vendor-supplied GPU libraries (e.g., NVIDIA CUDA \cite{cuda} and AMD HIP \cite{hip}) provide GPU multi-process services to manage GPU resource allocations (e.g. CUDA MPS and CUDA MIG \cite{MPS, MIG}) to concurrently execute kernels issued by the host device. Unfortunately, most popular edge GPUs are not supported with vendor-supplied hardware resource allocation tools due to architecture limitations. Meanwhile, although multi-stream mechanisms can help developers hide the latency of memory copy and support kernel overlapping, the contention problem still exists, also, the lack of stream management including unpredictable stream assignments would lead to an increasing tail latency of issued kernels. 

Efforts from the GPU community have been proposed to improve the overall throughput of the GPU system under multiple workloads. Warped-Slicer \cite{warpslicer} utilizes performance versus increasing computing unit occupancy curves to select an optimized simultaneous kernel pattern, which failed to address the contention between kernels. Works like HSM \cite{hsm} and \cite{wang2019efficient} model the latency degradation of concurrent GPU kernel executions based on hardware info. The predictors built in these works are hard to adapt to real-world multi-DNN inference because of the nondeterministic property of kernel overlapping \cite{enablesc}. Although works such as PACT \cite{kayiran2013neither} and \cite{iccd} try to fewer hardware resources such as threads to solve DRAM contention due to multi-workloads execution, these works are either focus on static workloads or not fully exploiting scheduling space. Other works \cite{smcentric, effisha} address the GPU multitasking problem from the resource management perspectives, either in a time-multiplexing manner \cite{infaas}, or space-multiplexing manner \cite{wu2020model,jain2019fractional}, which are orthogonal to our approach. 

Although our work is not the first work that demystifies kernel contention on edge GPU, Miriam focuses on multi-DNN workloads and first takes a holistic approach to exploit to solve both intra-SM and inter-SM contention based on parametric kernels with elastic launching mechanism and a dynamic kernel overlapping scheme at runtime in a lightweight manner, which differs from prior works.

==> overview.tex <==
\section{Miriam Overview} \label{overview}

Based on the above insights, we propose Miriam. The goal of Miriam is to provide high-throughput multi-DNN inference to achieve real-time for latency-critical DNN based tasks. Based on the insight that on-board DNN kernel contention is mainly rooted from intra- and inter- SM resource contention, Miriam provides three novel designs named MGen to automatically generate elastic GPU kernels based on equivalently transformation while supporting fine-grained control over SM-level resource utilization distribution, MPred to offline modeling the relationships between static analysis results of GPU kernels and the contention, which can assist the online coordination stage, MCoord to based on the wavefront DNN graph partition and resource-aware kernel group formation based on the most-room policy at runtime. Miriam jointly consider contention-inhibitors and contention-prohibitors to maximize the concurrency space of runtime multi-DNN inference and thus accelerate the tasks. The system overview of Miriam is shown in Fig. \ref{overview1}.

\subsection{Problem Formulation}
A Multi-DNN inference task is consist of multiple DNN model inference sub-tasks co-locating on one GPU device. Here we formulate the problem by fixing the number of co-running tasks as two for convenience, while the number can be extended.

During inference runtime, Miriam always holds two \textit{task queues} for each of these two models, in which is a series of kernels to be executed:
\begin{equation}
\begin{aligned}
T_{1}: [0,1,2...] \\
T_{2}: [0,1,2...]
\label{eq:seq}
\end{aligned}
\end{equation}
\noindent where each task queue is bound to a CUDA stream. The multi-stream mechanism can ensure the basic task-level concurrency. Kernels inside a task queue have data dependency and the order of them cannot be changed. To further mange the concurrency in a finer-grained manner. We insert \textit{sentinels} $se$, to manually split each task queue into smaller length, and include this sub-sequence of task queues from each DNN model into a "bin-packed" box, named \textit{kernel groups}. Miriam adopts a proactive scheduling sapience at runtime and hide the \textit{MCoord} running overhead by placing this module on CPU and hide its latency by co-execution with kernel inference tasks on GPU. For example, if we have $se_{1}$ as 2 and $se_{2}$ as 1, then the kernel group $G$ we form can be represented as:
\begin{equation}
\begin{aligned}
G:\{T_{1}[0,1,2]+T_{2}[0,1]]\}
\label{eq:kernel group}
\end{aligned}
\end{equation}
\textit{MCoord} proactively generates a schedule to coordinate the kernels in side each kernel group. Specifically, the schedule for each group $\pi $ is composed of two optimization knobs to be determined:
\begin{equation}
\begin{aligned}
\pi_{G}:\{\tau,\varphi\}
\label{eq:kernel group}
\end{aligned}
\end{equation}
where $\tau$ represents the policy of elastic version selection for each kernel, and $\varphi$ refers to the determination of overlapping. These two sub-schedules correspond to aforementioned \textit{contention in-
hibitors} and \textit{Contention Incentives}, which Miriam jointly considered with. Based on this, we can exploit a large on-device parallelism optimization space on edge GPU.
\begin{figure}[t!]%[htb]
\centering
\includegraphics[width=0.48\textwidth]{image_sysdesign/systemdesign.pdf}
\caption{Miriam Overview.}
\label{overview1}
\end{figure}
Finally, our system design target is to adaptively form the kernel group $ G$ at runtime and generates the corresponding schedule with the lowest latency. For each group $g$, the target can be represented:

\begin{equation}
\begin{aligned}
\Pi = argmin\Gamma(\pi_{g}), \pi\in\Pi \, \, \, \, \, s.t. \\ 
f(\pi_{g+1})<\Gamma(\pi_{g})
\end{aligned}
\end{equation}

where $\Pi$ is the optimal kernel coordination strategy, $f$ is the \textit{MCoord} running overhead for a kernel group on CPU, which is hided by the prior kernel group execution on GPU. $\Gamma$ refers to the execution latency measurement.

Fig. \ref{overview1} demonstrates the system goal: to coordinate both \textit{contention in-
hibitors} and \textit{Contention Incentives} optimization knobs for a generated kernel group.
\begin{figure}[t!]%[htb]
\centering
\includegraphics[width=0.2\textwidth]{image_sysdesign/1.pdf}
\caption{Generating a kernel group level scheduling.}
\label{overview2}
\end{figure}

%Architecture

%Formulation

==> pictures.tex <==
\section{Extra Figures} \label{pictures}

\begin{figure}[t!]%[htb]
\centering
\includegraphics[width=0.48\textwidth]{image_bk/mcoordNewNew.pdf}
\caption{Shaded Binary Tree for Kernel Shards Formations. The sharding degree represents the degree of elastic kernel splitting depth.}
\label{binary}
\end{figure}


\begin{figure}[t!]%[htb]
\centering
\includegraphics[width=0.48\textwidth]{image_bk/GPUruntimeExample.pdf}
\caption{GPU runtime in Miriam with a real kernel coordination example.}
\label{mcoordexample}
\end{figure}

==> related.tex <==

\section{Related Work} \label{related}
We compare and contrast Miriam with prior works in the following three aspects: on-device DNN inference serving, multi-DNN coordination system and multi-tasking on GPU.

\subsection{On-device DNN Inference Serving}
On-device DNN inference in full-stack can be roughly expanded in input data level, DNN kernel level, DNN model level, and hardware resource level. Works such as \cite{elf,edgeluyang} either adopts content-aware inputs selection mechanisms or heat-map-based processing of input streams algorithms to improve on-device inference efficiency; Model-level optimization has been extensively studied to exploit the sparsity of DNN models, e.g., iterative pruning \cite{lottery} and neural network search \cite{nas}; Kernel-level optimizations can be categorized into single-tenant DNN compiling techniques \cite{TVM,TASO}, which generate high-performance tensor programs inside each DNN kernel, or automatically find the optimal kernel fusion \cite{nimble} and parallelism strategy to accelerate the end-to-end DNN inference speed \cite{iosmlsys}. Some compiler-level works such as Rammer \cite{rammer} and TensorRT \cite{tensorrt} enable both inter- and intra-operator parallelism for accelerating DNN inference. Some recent works also exploit to utilize heterogeneous platforms \cite{dart, codl} e.g. mobile CPU \& GPU to boost inference performance. Dart \cite{dart} proposes a pipeline-based approach to co-run diverse DNN workloads on heterogeneous computation nodes. As mentioned, most of these works rapidly degrade under multi-DNN inference settings due to severe resource contention. Our work focuses on improving multi-DNN inference serving on a single edge GPU.
% Our work focuses on edge GPU, which have emerged as a popular accelerator to serve DNN inferences for edge computing applications \cite{gpu good}. As mentioned, directly running multiple DNN tasks concurrently on a single edge GPU will result in severe latency degradation which may exceed the QoS target set by users due to on-board resource contention.

\subsection{DNN Compiling}
Although most vendor-provided libraries such as NVIDIA cuDNN offer optimized DNN kernels with convenient APIs (e.g. $cudnn\_conv\_winograd$), many researchers have put their attention on DNN compilers, which automatically generate high-performance kernels which outperform those libraries. Although traditional DNN compilers such as IOS,  TVM and XLA \cite{iosmlsys,TVM,xla} have extensively explored either graph substitution based on inter-operator parallelism \cite{astitch} or kernel optimization \cite{rammer} based on intra-operator parallelism to boost inference speed. Unfortunately, they mainly target at optimizing one model under static environments, which is ill-fitted for mutli-DNN inference scenarios,s and give no consideration to on-device resource contentions on edge devices. For example, Auto-scheduler in Ansor \cite{ansor}, as Figure \ref{background1} shows, for a GEMM kernel on a RTX2060 GPU, the tuned configurations are aimed to saturate all SMs and memory bandwidth on the GPU, while these configurations can be sub-optimal when there are only partial resources available for the task when there comes another DNN task. The latency gap between single-model vs. multi-models with different tuned configurations can be X difference for a GEMM kernel. 

Readers may raise the question why not try leveraging DNN compilers to generate multiple versions of kernels under different contention levels, and adapt them online, switch the version of kernels in order to avoid resource contention? There are two main drawbacks of this kind of approach, current popular learning-based DNN compilers such as TVM search the optimal code transformation during compiling, leading to extremely long search time. For example, the time consumption for on-device measurements of a VGG16 model can be up to 10 hours on an NVIDIA TX2 \cite{moses}, which is unacceptable, not to say to generate multiple versions of a single kernel. Besides, pre-loading multiple versions of kernels into GPU will be a memory disaster. Thus, we cannot directly apply DNN compiler to solve the problem.

\subsection{Multi-DNN Coordination System}
A number of systematic solutions have been proposed in order to solve the on-device multi-DNN coordination problem, which can be divided into two categories: \textit{compression-enabled DNN inference system} and \textit{runtime operator scheduling system}. As for the prior one, works like NestDNN \cite{nestdnn} and RT-mDL \cite{rt-mdl} leverage DNN model compression techniques to provide a multi-variants design for each DNN model and to enable on-device multi-DNN inference acceleration by trading accuracy of each model at a modest level to exhaustively reduce the computation demands of the incoming mixed DNN workloads \cite{modelcompression}. There exist two main drawbacks: first, the compression ratio is task-dependent which makes the system less generality. Second, the model complexity-efficiency trade-off of these compressed models is determined in advance and is fixed after deploying them online, leading to rigid adaptiveness to varying runtime on-board resources. There are representative works for the second direction such as DeepEye \cite{deepeye}, Abacus \cite{enablesc} and Dart \cite{dart}. The key idea behind these works is to interleave operators with different "contention channels" (memory-bound or compute-bound) to avoid on-device resource contention, and thus to coordinate different DNN inference tasks. However, these works suffer from a time-consuming offline profiling process and are hard to generalize to new incoming DNN tasks. Above all, all these mentioned works can be described as \textit{"contention inhibitors"}, which deal with the multi-tasks on-device contention problems with an evasive attitude. Although it partially solves the contention by avoiding it, it would easily lead to resource under-utilization. Miriam consolidates both \textit{"contention inhibitors"} and \textit{"Contention Incentives"} to maximize on-device parallelism and minimize contention brought by multi-DNN inference on edge GPU.

\subsection{GPU Multi-tasking}
Current popular vendor-supplied GPU libraries (e.g., NVIDIA CUDA \cite{cuda} and AMD HIP \cite{hip}) provide GPU multi-process services to manage GPU resource allocations (e.g. CUDA MPS and CUDA MIG \cite{MPS, MIG}) to concurrently execute kernels issued by the host device. Unfortunately, most popular edge GPUs are not supported with vendor-supplied hardware resource allocation tools due to architecture limitations. Meanwhile, although multi-stream mechanisms can help developers hide the latency of memory copy and support kernel overlapping, the contention problem still exists, also, the lack of stream management including unpredictable stream assignments would lead to an increasing tail latency of issued kernels. 

Efforts from the GPU community have been proposed to improve the overall throughput of the GPU system under multiple workloads. Warped-Slicer \cite{warpslicer} utilizes performance versus increasing computing unit occupancy curves to select an optimized simultaneous kernel pattern, which failed to address the contention between kernels. Works like HSM \cite{hsm} and \cite{wang2019efficient} model the latency degradation of concurrent GPU kernel executions based on hardware info. The predictors built in these works are hard to adapt to real-world multi-DNN inference because of the nondeterministic property of kernel overlapping \cite{enablesc}. Although works such as PACT \cite{kayiran2013neither} and \cite{iccd} try to fewer hardware resources such as threads to solve DRAM contention due to multi-workloads execution, these works are either focus on static workloads or not fully exploiting scheduling space. Other works \cite{smcentric, effisha} address the GPU multitasking problem from the resource management perspectives, either in a time-multiplexing manner \cite{infaas}, or space-multiplexing manner \cite{wu2020model,jain2019fractional}, which are orthogonal to our approach. 

Although our work is not the first work that demystifies kernel contention on edge GPU, Miriam focuses on multi-DNN workloads and first takes a holistic approach to exploit to solve both intra-SM and inter-SM contention based on parametric kernels with elastic launching mechanism and a dynamic kernel overlapping scheme at runtime in a lightweight manner, which differs from prior works.
